Present status of PICOLON project

The existence of cosmic dark matter and neutrino properties are long-standing problems in cosmology and particle physics. These problems have been investigated by using radiation detectors. We will discuss the application of inorganic crystal scintillators to studies on dark matter and neutrino properties. A large volume and high-purity inorganic crystal is a promising detector for investigating dark matter and neutrino.

==> advantage.tex <==
\subsection{Radiation detectors for rare fundamental processes}
Various radiation detectors are applied to search for fundamental nuclear and particle physics.
Semiconductors are a significant advantage in their energy resolution and particle identification.
Their energy resolution is one of the most crucial properties, which enables a highly-sensitive confirmation of a small peak of \znu \ events.
Many groups simultaneously observe the ionization and phonon to identify the events.
The CDMS group applied Si semiconductors for WIMPs search \cite{CDMS2002}.
They observed both ionization and phonon, and the nuclear recoil events were identified from the raw data \cite{CDMS2002}.
They selected background events by investigating the position information in a Ge crystal \cite{CDMS2016}.

A liquid xenon scintillator is the world's most sensitive detector for dark matter and double-beta decay experiments.
XENON group developed a double-phase radiation detector that measures ionization, and scintillation \cite{AprileEpj2018, XENONnT2022}.
The liquid xenon detector has a significant advantage in its purity of the scintillation material. 
Purifying liquid xenon is done by distillation and filtration \cite{Aprile2022}.
They repeatedly remove radioactive contamination after they finish construction.
Consequently, the concentration of radioactive contamination will be kept sufficiently low during the experiment.

\subsection{Advantages of inorganic crystal scintillator}
Inorganic crystal scintillators present the following two challenges. The first is that it is difficult to confirm high purity, and the second is that the crystals require careful handling.

 To confirm the purification procedure, one must assemble and measure its radioactive contamination with a radiation detector.
The cost and time of crystallization, assembly, and low-background measurements are much less favorable than liquid xenon detectors.
 Especially for highly deliquescent crystals, such as NaI(Tl) crystals, the material used to seal them in the detector housing must also be of sufficiently high purity. 

If the purity of the raw material can be confirmed with sufficient accuracy, it is possible to avoid rebuilding the detector, effectively reducing costs. In recent years, the analytical accuracy of ICP-MS has been improving, making it possible to quantify impurities such as potassium, which used to be difficult to measure due to high interference. 
It is common practice to use ICP-MS to check the concentration of radioactive impurities in raw materials before manufacturing detectors for dark matter \cite{Park2020}.

Special care should be taken in handling the crystals because NaI(Tl) is highly cleavage prone, and the crystals are brittle. Furthermore, since NaI(Tl) is highly deliquescent, it is necessary to pay sufficient attention to the surrounding environment to prevent deliquescence during observation.
Preventing the crystals from cracking is possible by transporting the crystals to the laboratory on a sufficient anti-vibration table and preventing sudden temperature changes. There is no need to worry about deliquescence since the experiment is conducted under sufficiently low humidity conditions with dry nitrogen around the detector. PICOLON's NaI(Tl) uses an acrylic housing and shows no signs of tidal melting even after being in the shield for over three years.

The advantages of inorganic crystal scintillators are described below.
Inorganic crystals are stable and, therefore, extremely inexpensive to operate. They do not require constant cooling like liquid xenon or frequent security inspections like huge liquid scintillators.
Also, since no external impurities are introduced, the background can be maintained in a stable state. If the purity of the detector crystal is sufficiently improved, no further contamination will occur. The only challenge is with $^{226}$Ra and its progeny. Since this has a long half-life of $^{210}$Pb on the way, which is longer than the experimental period, there is concern that the number of $^{210}$Pb progeny will increase. However, since the radioactivity concentration of $^{226}$Ra has achieved less than 10~$\mu$Bq/kg
\cite{FushimiPTEP2020}, the amount of $^{210}$Pb will increase only 10~$\mu$Bq/kg at the maximum from the initial contamination amount. 

Inorganic scintillators have many options, including nuclei that are attractive targets for cosmic dark matter searches and double beta decay searches. For light WIMPs, CaF$_{2}$, CaI$_{2}$, and NaI, which contains nuclei with light masses, can be applied.
NaI, SrI$_{2}$, and CsI can be applied for those containing atoms with large atomic numbers for axion search.

For the double beta decay search, we have many selections as follows.
CaF$_{2}$ and CaI$_{2}$ containing $^{48}$Ca, CdWO$_{4}$ containing $^{116}$Cd, (Gd$_{2}$SiO5:Ce) and GAGG (Gd$_{3}$(Ga,Al)$_{5}$O$_{12}$:Ce) containing $^{160}$Gd,  and other promising scintillators are provided.

